Deep active learning for nonlinear system identification

The exploding research interest for neural networks in modeling nonlinear dynamical systems is largely explained by the networks' capacity to model complex input-output relations directly from data. However, they typically need vast training data before they can be put to any good use. The data generation process for dynamical systems can be an expensive endeavor both in terms of time and resources. Active learning addresses this shortcoming by acquiring the most informative data, thereby reducing the need to collect enormous datasets. What makes the current work unique is integrating the deep active learning framework into nonlinear system identification. We formulate a general static deep active learning acquisition problem for nonlinear system identification. This is enabled by exploring system dynamics locally in different regions of the input space to obtain a simulated dataset covering the broader input space. This simulated dataset can be used in a static deep active learning acquisition scheme referred to as global explorations. The global exploration acquires a batch of initial states corresponding to the most informative state-action trajectories according to a batch acquisition function. The local exploration solves an optimal control problem, finding the control trajectory that maximizes some measure of information. After a batch of informative initial states is acquired, a new round of local explorations from the initial states in the batch is conducted to obtain a set of corresponding control trajectories that are to be applied on the system dynamics to get data from the system. Information measures used in the acquisition scheme are derived from the predictive variance of an ensemble of neural networks. The novel method outperforms standard data acquisition methods used for system identification of nonlinear dynamical systems in the case study performed on simulated data.

==> archive/deleted_text.tex <==
 \begin{comment}
 
 
 \begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{heat_transf_cond_conv.pdf}
    \caption{Convection and conduction trough several materials}
    \label{fig:conv_cond_heat_trans}
\end{figure}
Figure \ref{fig:conv_cond_heat_trans} illustrates heat being transferred from left to right from a fluid, through a planar wall consisting of two different solid materials, and to a second fluid. The heat is transferred through a cross-section area $A$. The fluid on the right has a heat transfer coefficient $h_1$, and a bulk temperature of $T_{f1}$. The solid material to the left has conductivity $k_1$ and thickness $x_1$. Furthermore, the temperature on the left boundary of the solid materials is $T_1$, and the temperature between the two solid materials is $T_2$. The conductivity of the solid material to the right is $k_2$ and the thickness of this material is $x_2$. The temperature of the right edge of the right material is $T_3$. The fluid to the right has a heat transfer coefficient of $h_2$, and the bulk temperature of this fluid is $T_{f2}$. Note that $T_{f1} > T_1 > T_2 > T_3 > T_{f2}$.
Heat transferred from the left fluid to the left boundary of the solid material is given by:
\begin{equation}
    Q_1 = h_1 \cdot A \cdot (T_{f1} - T_1),
\end{equation}
heat transferred through the left solid material is given by:
\begin{equation}
    Q_2 = k_1 \cdot A \cdot \frac{T_1 - T_2}{x_1},
\end{equation}
heat transferred through the right solid material is given by:
\begin{equation}
    Q_3 = k_2 \cdot A \cdot \frac{T_2 - T_3}{x_2},
\end{equation}
and heat transferred from the edge of the right wall to the fluid at the right side is given by:
\begin{equation}
    Q_4 = h_2 \cdot A \cdot (T_{3} - T_{f2}).
\end{equation}
If it is assumed that heat flow is steady state, the heat flow through each thermal resistor are assumed equal:
\begin{equation}
    Q_1 = Q_2 = Q_3 = Q_4 = Q
\end{equation}
Assuming steady heat transfer, the heat transfer in Figure \ref{fig:conv_cond_heat_trans} would be modeled as:
 \begin{equation}
     Q = \frac{T_{f1} - T_{f2}}{1/(h_1\cdot A) + x_1/(k_1 \cdot A) + x_2/(k_2 \cdot A) + 1/(h_2 \cdot A)}.
 \end{equation}
\end{comment}

==> archive/sim_mod.tex <==
\section{Simulation model}
In this section we will follow a purely physics-based approach to deriving the equations. At appropriate places we will highlight the challenges and assumption 

The dynamical system simulated in this study is generated by the set of ordenary differential equations (ODE's) in equation (\ref{eq:xdot1}) - (\ref{eq:xdot8}). This system of equations is derived from a simplified model of an aluminum electrolysis cell. This model comprises simplified energy and mass balance of the electrolysis cell. The model consider an energy balance based on sideways heat transfer, energy transfer between side ledge and bath due to melting and freezing of cryolite, and energy input as a function of electrical resistance in the electrolyte and voltage drop due to bubbles. The mass balance includes mass transfer between side ledge and bath, input of $Al_2O_3$ and $AlF_3$, production of metal and consumption of the raw material $Al_2O_3$ and tapping of metal from the electrolysis cell.  In table \ref{table:states_inputs}, the system states and inputs are described. The purpose of the simulation model is not to mimic the exact dynamics of an aluminum electrolysis cell, but rather to generate nonlinear dynamics similar to what occurs in a real aluminum electrolysis. 


\subsubsection{Heat capacity}
Heat capacity is a measure of the amount of thermal energy a body of a certain material can store for a given temperature and volume and is given by the definition \cite{gale2003smithells}:
\begin{equation}
    C = \frac{\delta q}{\delta T}.
\end{equation}
$C [J/^\circ C]$ is the heat capacity, $\delta q [J]$ is an infinitesimal heat quantity and $\delta T [^\circ C]$. Specific heat capacity $c_p$ is heat capacity at constant pressure per unit of mass:
\begin{equation}
    c_p = \left(\frac{d h}{d T}\right)_p,
\end{equation}
where $c_p \; [J/(kg ^\circ C]$ is the specific heat capacity, $h \; [J/kg]$ is specific enthalpy and $T \; [^\circ C]$ is temperature. The subscript $p$ indicates constant pressure. In the process of aluminum electrolysis, the pressure can be assumed to be constant at $p = 1 \;[atm]$. 

\subsubsection{Energy and mass balance}
The first law of thermodynamics known as the energy conservation principle states the following \cite{dincer2014advancedpower}:
\begin{equation}
    \frac{d E_{i}}{d t} = \Dot{E}_{in, \; i} - \Dot{E}_{out, \; i}.
\end{equation}
$\frac{d E_{i}}{d t} \; [W]$ is the change of energy of species $i$ in the system, $\Dot{E}_{in, \; i} \; [W]$ is the energy input rate and $\Dot{E}_{out, \; i} \; [W]$ is the energy output rate of species $i$ the system. System is here used synonymous to control volume. The energy of the system can be transferred through heat, work or through the energy associated with the mass crossing the system boundary. This can be expressed as follows:
\begin{eqnarray}
    \Dot{E}_{in, \; i} &=&  \Dot{Q}_{in, \; i} +  \Dot{W}_{in, \; i} + \Dot{m}_{in, \; i}e_{in, \; i}\\
    \Dot{E}_{out, \; i} &=&  \Dot{Q}_{out, \; i} + \Dot{W}_{out, \; i} + \Dot{m}_{out, \; i}e_{out, \; i}
\end{eqnarray}
    where $\Dot{Q}_{in, \; i} \; [W]$ and $\Dot{Q}_{out, \; i}\; [W]$ are the rates of heat in and out of the system and $\Dot{W}_{in, \; i} \; [W]$ and $\Dot{W}_{out, \; i} \; [W]$ is the rate of work generated on the system. $\Dot{m}_{in, \; i} \; [kg/s]$ and $\Dot{m}_{out, \; i}\; [kg/s]$ is the mass rate into the system and out of the system respectively, whereas $e_{in, \; i}\; [J/kg]$ and $e_{out, \; i}\; [J/kg]$ is the specific energy of the mass entering and leaving the system. The specific energy can be formulated as:
    \begin{equation}
        e = u + \frac{1}{2}v^2 + gz,
    \end{equation}
    where $u \; [J/kg]$ is the specific internal energy, $\frac{1}{2}v^2 \; [J/kg]$ is the specific energy related to velocity $v \; [m/s]$, and $gz \; [J/kg]$ is the specific energy related to elevation difference $z \; [m]$. 
    
    The change of system energy $ \frac{d E_{i}}{d t} = \Dot{E}_{i}$ can be written as:
    \begin{equation}
        \frac{d E_{i}}{d t} = \frac{d (m_{i}e_{i})}{d t},
    \end{equation}
where $m \; [kg]$ is the mass of the system and $e_{i} \; [J/kg]$ is the specific energy of the system. Since the relevant control volumes are related to an aluminum electrolysis, it is reasonable to neglect the terms $\frac{1}{2}v^2$ and $gz$. In this work, $\Dot{Q} = Q_{in, \; i} - Q_{out, \; i}$ is defined as positive when net heat is provided to the system, and $W = W_{in, \; i} - W_{out, \; i}$ is positive when work is added to the system. Thus, the resulting energy equation can be formulated as:
\begin{equation}
    \frac{d(m_{i}u_{i})}{dt} = m\frac{d u_{i}}{dt} + u_{i}\frac{dm_{i}}{dt} =\Dot{m}_{in, \; i}u_{in, \; i} - \Dot{m}_{out, \; i}u_{out, \; i} + \Dot{Q} + \Dot{W}.
\end{equation}
Work $W\; [J]$ is organized transfer of energy. $W$ can be divided into several types of work \cite{skogestad2008chemical}:
\begin{equation}
    W = W_{flow} + W_{\Delta V} + W_s + W_{el} + W_{other}.
\end{equation}
$W_{flow}$ is the work associated with the volume displacements of streams that enter and exit the system, $ W_{\Delta V}$ is the work associated with changes of the volume of the system, $W_s$ is the mechanical work supplied using movable machinery, $W_{el}$ is the electrochemical work supplied when the system is connected to an external electric circuit. $W_{other}$ is the sum of other types of work, for example if surface areas changes or electromagnetic work. For an aluminum electrolysis, $W_{\Delta V} = W_s = W_{other} \approx 0 $. $W_{flow}$ is given by:
\begin{equation}
    W_{flow} = pV,
\end{equation}
where $p$ is pressure and $V$ is volume. Enthalpy $H \; [J]$ is given by:
\begin{equation}
    H = U + pV.
\end{equation}
where $U = m\cdot u \;[J]$. Furthermore, $H = h\cdot m$. Thus:
\begin{equation}
     m\frac{d u_{i}}{dt} + u_{i}\frac{dm_{i}}{dt} = \Dot{m}_{in, \; i}h_{in, \; i} -\Dot{m}_{out, \; i}h_{out, \; i} + \Dot{Q} + \Dot{W}_{el}.
\end{equation}
Assuming that the flow work is neglectable compared to the other quantities in the energy equation for aluminum electrolysis gives that $H \approx U$. Recall that $c_p = \frac{d h}{d T}$. Hence:
\begin{equation}
     \frac{d u_{i}}{dt} \approx \frac{d h_{i}}{dt} = \frac{\partial h_{i}}{\partial T_{i}}\frac{d T_{i}}{dt} = c_{p_{i}} \frac{d T_{i}}{dt},
\end{equation}
where $\frac{dT}{dt} = \Dot{T_{i}} \; [^\circ T]$ is the temperature derivative with respect to time. This yields:
\begin{equation}
    \frac{dT_{i}}{dt} = \frac{1}{m_{i} c_{p_{i}}}\left(\Dot{m}_{in, \; i}h_{in, \; i} - \Dot{m}_{out, \; i}h_{out, \; i} + \Dot{Q} + \Dot{W_{el}} - u_{i}\frac{dm_{i}}{dt}\right) 
\end{equation}
The mass rate equation can be formulated as:
\begin{equation}
    \frac{d m_i}{dt} = \Dot{m}_{in} - \Dot{m}_{out} + \sum_{j=1}^{n_j}r_{i,j},
    \label{eq:mass_rate_eq}
\end{equation}
where $r_{i,j}$ is the reaction rate of species $i$ being produced or consumed in reaction $j$. Assuming that the contents of the control volume to be perfectly mixed and assuming that the flow work is neglectable gives:
\begin{equation}
    u_i \approx h_i = h_{out, \; i}.
\end{equation}
Hence, the resulting temperature specific energy equation for component $i$ in a control volume is given by:
\begin{equation}
    \frac{d T_{i}}{dt} = \frac{1}{m_i c_{p_i}}\left(\Dot{m}_{in,i}(h_{in, i} - h_{out,i}) + \Dot{Q} + \Dot{W}_{el} - h_{out, \; i} \sum_{j=1}^{n_j}r_{i, \; j}.    \right)
    \label{eq:comp_temp_derivatives}
\end{equation}
The latter equation states that the time derivative of the temperature in the control volume is dependent on the composition of species in the control volume. It is assumed that the temperature is equal for all components in the control volume. Furthermore, it is assumed that there is a common heat loss $\Dot{Q}$ from a control volume to other control volumes, and that electrical power $\Dot{W}_{el}$ is performed on the whole control volume instead of on different components in the control volume. When different components are mixed in a control volume, the enthalpy of this mix is more complex than adding the enthalpy of individual species. However, the complexity of mixed enthalpy is left out of this simulation model. The heat capacity of a mix of components in a control volume $c_{p_{cv}}$ is simplified to be constant despite of that $c_{p_{cv}}$ varies with composition and temperature in the control volume. The values for different species and control volumes are taken from \cite{TAYLOR1996913} and \cite{drengstig1997process}.
Thus, the simplified simulation equation for the temperature derivative in a control volume is given by:  
\begin{equation}
    \frac{d T_{cv}}{dt} = \frac{1}{m_{cv} c_{p_{cv}}}\left( \left[\sum_{i=1}^{n_i}\Dot{m}_{in,i}(h_{in, i} - h_{out,i})\right] + \Dot{Q} + \Dot{W}_{el} - \sum_{i=1}^{n_i}\left[h_{out, \; i} \sum_{j=1}^{n_j}r_{i, \; j}\right]\right),
    \label{eq:general_temp_derivatives}
\end{equation}
where $m_{cp}$ is the sum of masses in the control volume.

\subsubsection{Heat transfer}
Heat transfer $\Dot{Q} [W]$ will from this point be referred to as $Q$, meaning that the dot is omitted. the In the process of aluminum electrolysis, the two most important principles for heat transfer are convection and conduction. \textbf{Conduction} is heat transfer through molecular motion within a solid material. The expression for conduction is given by
\begin{equation}
    Q = -k\cdot A \cdot \frac{\partial T}{\partial x}.
\label{eq:conduction_Fourier}
\end{equation}
 $Q \; [W]$ is heat transferred,  $A \; [m^2]$ is the area the heat is transferred through $\frac{\partial T}{\partial x} \; [^\circ C/m]$ is the temperature gradient in the direction $x$ that the heat is transferred, and $k \; [W/(m ^\circ C)]$ is the thermal conductivity, a material dependent proportionality constant. For a fixed cross-section area, the one dimensional \textbf{steady state heat flow} through a wall of thickness $x\; [m]$ from $x=0$ with temperature $T_1$ to $x=1$ with temperature $T_1$ integrates to:
 \begin{equation}
     Q = k \cdot A \cdot \frac{T_1 - T_2}{x},
 \end{equation}
 where $T_1>T_2$. Thermal conductive resistance for a plane wall can be extracted from the latter expression:
 \begin{equation}
     R_{cond} = \frac{x}{k\cdot A},
 \end{equation}
 where $R_{cond} [^\circ C/ W]$ is the thermal resistance,  $x[m]$ is the thickness of the solid material in the direction heat is transferred, and $k$ and $A$ are as mentioned above. Thermal conductive analysis is analogous to an electrical circuit, where the temperature difference is analogous to the potential difference $V$, the heat flow is analogous to the electrical current $I$ and thermal resistance is analogous to electrical resistance $R_{el}$. 
\textbf{Convection} is the heat transfer through the mass motion of a fluid. Heat transfer between a surface at temperature $T_s$ and a fluid at a bulk temperature $T_f$ is due to convection.  Convection can be formulated as:
 \begin{equation}
     Q = h \cdot A \cdot(T_s - T_f),
 \end{equation}
 where $A [m^2]$ is the contact surface between a solid surface and the liquid, the the heat transfer coefficient $h \; [W/(m^2) ^\circ C]$ is the proportionality constant between the heat flux and the thermodynamic driving force for the flow of heat, i.e. the temperature difference $(T_s - T_f)$. 
 
 
 
Thermal resistance can be defined for a fluid $R_{conv}$, and is given by:
 \begin{equation}
     R_{conv} = \frac{1}{h \cdot A}.
 \end{equation}
 
 As for electrical circuits, thermal resistances can be coupled in series, and the reciprocal of the total resistance equals the sum of reciprocals of individual resistances:
 \begin{equation}
     \frac{1}{R_{tot}} =\sum_{i=1}^N \frac{1}{R_i}
     \label{eq:term_resist_series}
 \end{equation}
Equation (\ref{eq:term_resist_series}) together with the assumption of stationary heat transfer makes it possible to calculate the heat transfer from one edge to the other through several resistors in series as the temperature difference between the edges divided by the sum of reciprocals of individual resistors:
 \begin{equation}
     Q = \frac{T_{1} - T_{N+1}}{\sum_{i=1}^N R_i}, 
     \label{eq:resist_series}
 \end{equation}
 where $T_1>T_2> ...>T_{N+1}$ is temperature and $R_i$ are the resistors. 
In the simulation model, the heat transfer is assumed to be piecewise stationary, meaning that the heat transfer is assumed to be constant from the middle of one control volume to the middle of the adjacent control volume. However, the heat transfer is not assumed to be stationary through several control volumes. Thus, there are separate energy balances for each control volume. Heat transfer is only considered through the side walls of the electrolysis cell. 

  \begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/thermo_CV_sim_mod.pdf}
    \caption{Convection and conduction trough several materials}
    \label{fig:conv_cond_heat_trans}
\end{figure}
Convective heat transfer $Q_{bath-liq}$ from the bath to the surface of the side ledge
\begin{equation}
    Q_{bath-liq} = h_{bath-sl}A_{sl}(T_{bath} - T_{liq}).
    \label{eq:Q_b_l}
\end{equation}
Conductive transfer $Q_{liq-sl}$ from surface of side ledge to the center of the side ledge
\begin{equation}
    Q_{liq-sl} = \frac{2k_{sl}A_{sl}(T_{liq} - T_{sl})}{x_{sl}}.
    \label{eq:Q_l_sl}
\end{equation}
Conductive heat transfer $Q_{sl-wall}$ from center of side ledge to the center of the side wall 
\begin{equation}
    Q_{sl-wall} = \frac{A_{sl}(T_{sl} - T_{wall}
    )}{(x_{wall}/2k_{wall}) + (x_{sl}/2k_{sl})}
\end{equation}
The heat transfer from the middle of the wall to the ambient $Q_{wall-0}$ consists of conductive heat transfer from the middle of the wall to the surface of the wall, and the convection from the surface of the wall to the ambient air
\begin{equation}
    Q_{wall-0} = \frac{A_{sl}(T_{wall} - T_0)}{(1/h_{wall-0}) + (x_{wall}/2k_{wall})}.
\end{equation}

\subsubsection{Electrochemical power}
Electrochemical power $\Dot{W}_{el} \; [W]$, from now referred to as $P_{el}$ is the amount of energy transferred to a system from a electrical circuit and is defined as:
\begin{equation}
    P_{el} = U_{cell} \cdot I_{line},
\end{equation}
where $U_{cell} \; [V]$ is the applied cell voltage and $I_{line} \; [A]$ is the line current sent through the electrolyte. The cell voltage is composed of three different types of voltage contributions. these are the \textbf{decomposition voltage}, which is the theoretical minimum potential for the decomposition of alumina, \textbf{overvoltage}, meaning the excess voltage  due to electrode polarization and \textbf{ohmic voltage drops}, due to resistance of various sections in the cell \cite{jessen2008mathematical}. These contributions can be divided into smaller contributions caused by different effects in different parts of the cells. To make the mathematical expression in the resulting nonlinear simulation model less comprehensive, only \textbf{ohmic voltage drop} contributions are included. These are:
\begin{itemize}
    \item Electrolyte voltage drop $U_{el} \; [V]$
    \item Bubble voltage drop $U_{bub}\; [V]$
\end{itemize}
The \textbf{voltage drop over the electrolyte} is due to the electrical resistivity of the electrolyte. Assuming uniform current density, the resistance of the elecrolyte is given by:
\begin{equation}
    R_{el} = \frac{1}{\kappa}\frac{d}{A}.
\end{equation}
$R_{el} \; [\Omega]$ is the electrical resistance, $\kappa \; [1/(\Omega m)]$ is electrical conductivity, $d \; [m]$ is the interpolar distance and $A \; [m^2]$ is the total surface of the anodes. The expression for electrical conductivity is given by \cite{grjotheim1993introduction}:
\begin{align}
    \kappa &=\, exp\biggl(2.0156 - \frac{2068.4}{T_{bath} + 273} + 0.4349\cdot BR - 2.07C_{al_2O_3} - 0.5C_{CaF_2} \nonumber \\
    &\,- 1.66 C_{MgF_2} + 1.78C_{LiF} + 0.77C_{Li_3AlF_6}   \biggr).
\end{align}
$T_{bath} \; [^\circ C]$ is the temperature of the electrolyte, $BR \; [-]$ is the bath ratio, while $C_{x} [-]$ is the concentration of substance $x$. $BR$ is assumed to be constant at $1.2$, $C_{MgF_2} = 0.01$, $C_{CaF_2} = 0.05$, $C_{LiF} = 0$ and $C_{Li_3 AlF_6} = 0$. Thus, $\kappa$ can be simplified to: 
\begin{equation}
    \kappa = exp\biggl( 2.496 - \frac{2068.4}{T_{bath} + 273} - 2.07C_{Al_2O_3}\biggr).
    \label{eq:el_cond}
\end{equation}
The voltage drop due to resistance in the electrolyte is given by:
\begin{equation}
    U_{EL} = R_{EL}\cdot I_{line}
\end{equation}
Gas accumulation beneath the anode surface which reduces the cross-sectional area of the electrolyte in that zone. Thus, the effective resistivity increases and causes the so called\textbf{ bubble voltage drop} $U_{bub}$ \cite{hyde1997gas}:
\begin{equation}
    U_{bub} = \frac{d_{bub} \cdot j_A}{\kappa}\frac{\phi}{1-\phi}.
\end{equation}
$j_A \; [A/cm^2]$ is the anode current density $d_{bub} \; [cm] $ in the bubble layer thickness and $\phi \; [-] $ is the bubble coverage as a fraction of the anode:
\begin{equation}
    d_{bub} = \frac{0.5517 + j_A}{1 + 2.167j_A},
    \label{eq:d_bub}
\end{equation}
and
\begin{align}
    \phi &=\, 0.509 + 0.1823j_A - 0.1723j_A^2 + 0.05504j_A^3 \nonumber\\
    &\,+ \frac{0.4322 - 0.3781BR}{1-1.637BR} + \frac{0.431 - 0.1437(x_{Al_2O3} - x_{Al_2O3}^{AE})}{1 + 7.353(x_{Al_2O3} - x_{Al_2O3}^{AE})}
    \label{eq:bub_cov}
\end{align}
$x_{Al_2O_3} \; [-]$ is the weight percent of alumina in the bath and $x_{Al_2O_3}^{AE} \; [-]$ is the weight percent of alumina at where the anode effect occurs, in this case it is assumed that $x_{Al_2O_3}^{AE} = 2.0$. Since the simulation model is simplified to only include contributions from $U_{bub}$ and $U_{EL}$, the total applied cell voltage in the simulation model is given by:
\begin{equation}
    U_{cell} = U_{EL} + U_{bub}.
\end{equation}

\subsubsection{Mass rates}
The substances considered in the simulation model are alumina ($Al_2O_3$), aluminum fluoride ($AlF_3$) and cryolite ($Na_3AlF_6$) in the bath and liquid aluminum ($Al$) in the metal pad below the bath. Aluminum is extracted from alumina, which is dissolved in the electrolytic bath. In addition to alumina, carbon anodes are consumed in the net reaction, producing molten aluminum and carbon dioxide gas ($CO_2$):
\begin{equation}
    2Al_2O_3 + 3C \rightarrow 3CO_2 + 4Al.
    \label{eq:primary_reac}
\end{equation}
This reaction occurs at a rate according to Farraday's law for aluminum electrolysis \cite{drengstig1997process}:
\begin{equation}
    r_{al} = \frac{CE \cdot I_{line}}{z\cdot F},
\end{equation}
where $r_{al} \; [mol/s]$ is the reaction rate of the primary reaction of the Hall-H\'eroult process presented in equation (\ref{eq:primary_reac}), $z=12$ is the number of electrones in the reaction, $F = 96486.7 [(A\cdot s)/mol]$ is the Faraday constant, and $CE [-]$ is the current efficiency, assumed constant at $CE = 0.95$. Feeded alumina contains several impurities \cite{drengstig1997process}. In the simulation model derived used in this work, only sodium oxide ($Na_2O$) is considered as additions in the feeded alumina. The content of $Na_2O$ in alumina react as:
\begin{equation}
    3Na_2O + 4AlF_3 \rightarrow 2Na_3AlF_6 + Al_2O_3.
    \label{eq:reac_bath_prod}
\end{equation}
$3$ Mol $Na_2O$ reacts with $4$ Mol of $AlF_3$ and produces $2$ Mol of $Na_3AlF_6$ and $1$ Mol of $Al_2O_3$. The reaction rate of the latter reaction $r_{bath} \; [kmol/s]$ can be formulated as:
\begin{equation}
    r_{bath} = \frac{C_{Na_2O}}{3 M_{Na_2O}}u_{Al_2O_3},
\end{equation}
where  $C_{Na_2O} \; [-]$ is the weight percent of $Na_2O$ in the alumina feed, $M_{Na_2O} \; [g/mol]$ is the molar mass of $Na_2O$ and $u_{Al_2O_3} \; kg/s$ is the rate of alumina feed. The reaction in equation (\ref{eq:reac_bath_prod}) affect the mass balance of both $AlF_3$, $Na_3AlF_6$ and $Al_2O_3$. Therefore, $r_{bath}$ is included in the mass balance equations of all these species. The general mass rate equation (\ref{eq:mass_rate_eq}) is used in the derivation the mass rate of side ledge, cryolite, alumina, aluminum fluoride and metal. The control volumes in which there are nonzero mass rates are the bath/electrolyte, the metal pad and the side ledge. The \textbf{mass rates in the electrolyte} are:
\begin{equation}
    \Dot{m}_{Al_2O_3} = (1 - C_{Na_2O})u_{Al_2O_3} - \frac{2}{1000}r_{al}M_{Al_2O_3} + r_{bath}M_{Al_2O_3}.
\end{equation}
$\Dot{m}_{Al_2O_3} \; [kg/s]$ is the mass rate of alumina and $M_{Al_2O_3} \; [g/mol]$ is the molar mass of alumina. $\frac{2}{1000}r_{al}M_{Al_2O_3} \; [kg/s]$ is the reaction rate of alumina produced due to the reaction in equation (\ref{eq:primary_reac})  and $r_{bath}M_{Al_2O_3} \; [kg/s]$ is the reaction rate of alumina due to the reaction in equation (\ref{eq:reac_bath_prod}). The mass rate of $AlF_3$ is given by:
\begin{equation}
    \Dot{m}_{AlF_3} = u_{AlF_3} - 4r_{bath}M_{AlF_3},
\end{equation}
where $\Dot{m}_{AlF_3} \; [kg/s]$ is the mass rate of aluminum fluoride, $u_{AlF_3} \; [kg/s]$ is the input rate of aluminum flouride and $4r_{bath}M_{AlF_3} \; [kg/s]$ is the reaction rate of produced aluminum fluoride from the reaction in equation (\ref{eq:reac_bath_prod}). The mass rate of cryolite in the bath is given by:
\begin{equation}
    \Dot{m}_{cry} = w_{fus} + 2r_{bath}M_{cry}.
\end{equation}
$\Dot{m}_{cry} \; [kg/s]$ is the mass rate of cryolite in the electrolyte, $ 2r_{bath}M_{cry} \; [kg/s]$ is the reaction rate of produced cryolite due to the reaction in equation (\ref{eq:reac_bath_prod}) and $w_{fus} \; [kg/s]$ is the mass rate of cryolite transferred between the side ledge and the bath. $w_{fus}$ is given by:
\begin{equation}
    w_{fus} = \frac{Q_{bath-liq} - Q_{liq-sl}}{\Delta_{fus}H_{cry}}.
\end{equation}
$Q_{bath-liq}$ and $Q_{liq-sl}$ is given in equation (\ref{eq:Q_b_l}) and (\ref{eq:Q_l_sl}) respectivelym and $\Delta_{fus}H_{cry}$ is the heat of fusion for cryolite, i.e. the amount of energy required to melt one $kg$ of cryolite. The heat of fusion for cryolite at $1000^\circ C$ is $\Delta_{fus}H_{cry} = 119495 \; [J/kg]$ \cite{drengstig1997process}, and is assumed to be constant in the simulation model. The \textbf{side ledge} is necessary to withstand the highly corrosive molten cryolite in the oven. The side ledge consists of \textit{frozen} cryolite \cite{drengstig1997process}. The mass rate of side ledge is therefore the transfer of cryolite between the electrolyte and side ledge due to melting and freezing:
\begin{equation}
    \Dot{m}_{sl} = - w_{fus}.
\end{equation}
$\Dot{m}_{sl} \; [kg/s]$ is the mass rate of side ledge, and $w_{fus} \; [kg/s]$ is given above. The \textbf{mass rate of aluminum} is given by:
\begin{equation}
\Dot{m}_{Al} = \frac{2}{1000}r_{al}M_{Al} - u_{tap}.
\end{equation}
$\Dot{m}_{Al} \; [kg/s]$ is the mass rate of aluminum, $\frac{2}{1000}r_{al}M_{Al} \; [kg/s]$ is the reaction rate of produced aluminum due to the reaction in equation (\ref{eq:primary_reac}), and $u_{tap} \; [kg/s]$ is the control input of tapping metal from the oven. 

\subsubsection{Temperature derivatives}
Equation (\ref{eq:general_temp_derivatives}) is used to calculate the temperature derivatives in the electrolyte, side ledge and side wall. As menitoned above, $\Dot{Q}  = Q$ and $\Dot{W}_{el}=P_{el}$. In the \textbf{electrolyte}, the energy is transferred in and out of the control volume in many different ways. Heat $Q_{bath-sl}$ is tranferred through convection from the bath to the side ledge surface ($Q_{bath-liq}$) and from the side ledge surface to the center of the side ledge with conductive heat $Q_{liq-sl}$. The resulting heat transfer can be formulated as:
\begin{equation}
    Q_{bath-sl} = \frac{T_{bath} - T_{sl}}{(x_{sl}/2k_{sl}A_{sl}) + 1/(h_{bath-sl}A_{sl})}.
\end{equation}
Energy is transferred through mass transfer in several ways. Energy needed to heat and melt substances fed as control input $u$ is given by:
\begin{equation}
    E_{u} = \Delta_{fus}H_{Al_2O_3}u_{Al_2O_3} + \Delta_{fus}H_{AlF_3}u_{AlF_3} + (T_{bath} - T_{in})(\Bar{c}_{p_{Al_2O_3}}u_{Al_2O_3} + \Bar{c}_{p_{AlF_3}}u_{AlF_3}). 
\end{equation}
$\Delta_{fus}H_{i} \; [J/kg]$ is the specific heat of fusion for substance $i$, and $\Bar{c}_{p_i} \; [J/(^\circ C kg)]$ is the average heat capacity from $T_{in}$ to $T_{bath}$.
Energy is also transferred through mass transfer between the electrolyte and the side ledge. When side ledge (frozen cryolite) melts into the bath, energy is required both to heat and melt the frozen cryolite. The energy required to heat the frozen cryolite is:
\begin{equation}
    E_{tc, \; liq} = w_{fus}c_{p,cry, liq}(T_{bath} - T_{liq}).
\end{equation}
$w_{fus} \; [kg/s]$ is as mentioned above the mass rate of cryolite between bath and side ledge, and is positive when cryolite melts and is transferred to the bath. $c_{p,cry, liq} \; [J/(^\circ C kg)]$ is the heat capacity of molten cryolite $T_{bath} \; [^\circ C]$ is the bath temperature and $T_{liq} \; [^\circ C]$ is the liquidus temperature at which cryolite melts and freezes. $E_{tc, \; liq} \; [W]$ is the energy required to heat molten cryolite from liquidus temperature to bath temperature. The subscript $tc$ stands for temperature change and the subscript $liq$ indicates that the substance is liquid. When $E_{tc, liq}$ is positive, it is becauce $W_{fus}$ is positive, indicating that cryolite is melting. Thus, when $E_{tc, liq}$ is negative, cryolite is freezing. The energy needed to melt frozen cryolite is given by:
\begin{equation}
    E_{sc} = w_{fus}\Delta_{fus}H_{cry}. 
\end{equation}
$E_{sc} \; [W]$ is the energy required to melt the mass of frozen electrolyte. The subscript $sc$ stands for state change, meaning that it transitions between solid and liquid. $\Delta_{fus}H_{cry} \; [J/kg]$ is the heat of fusion for cryolite as mentioned above. When $E_{sc}$ is positive, cryolite is melted and energy is required whereas when $E_{sc}$ is negative, cryolite freezes, and energy is released. Energy is required for the primary reaction in equation (\ref{eq:primary_reac}) since it is endothermic:
\begin{equation}
    E_{r_{al}} = r_{al}\Delta H_{r_{al}}.
\end{equation}
$E_{r_{al}} \; [W]$ is the amount of energy required for the reaction to take place, $r_{al} [mol/s]$ is as mentioned above the reaction rate of the primary reaction in the process, and $\Delta H_{r_{al}} =2197582\; [J/mol]$ is the enthalpy of reaction for (\ref{eq:primary_reac}). Since the reaction in 
equation (\ref{eq:reac_bath_prod}) is exothermic, this reaction releases energy to its surroundings. This is given by:
\begin{equation}
    E_{r_{bath}} = 1000r_{bath}\Delta H_{r_{bath}}.
\end{equation}
$E_{r_{bath}} \; [W]$ is the energy released due to the reaction in (\ref{eq:reac_bath_prod}) $r_{bath} \; [kmol/s] = 1000[mol/s]$ is the reaction rate of (\ref{eq:reac_bath_prod}) and $\Delta H_{r_{bath}} = -993283 \; [J/mol]$ is the entalpy of reation for (\ref{eq:reac_bath_prod}).
The time derivative for the bath temperature is given by:
\begin{equation}
    \Dot{T}_{bath} = \frac{P_{el} - Q_{bath-sl} - E_u - E_{tc, \; liq} - E_{sc} - E_{r_{al}} - E_{r_{bath}}}{m_{bath} c_{p_{bath, \; liq}}}.
    \label{eq:T_dot_bath}
\end{equation}
$m_{bath} \; [kg]$ is the mass of the liquid bath and $c_{p_{bath, \; liq}} \; [J/(^\circ C \cdot kg)]$ is the enthalpy of the liquid bath.  For the \textbf{side ledge} control volume, the energy transfer is through melting and freezing of cryolite and heat transfer. The energy transfer related to melting and freezing of cryolite is given by:
\begin{equation}
    E_{tc \; sol} = w_{fus}c_{p_{cry, \; sol}}(T_{liq} - T_{sl}).
\end{equation}
$E_{tc \; sol} \; [W]$ is the energy required into the side ledge when frozen cryolite heats from side ledge temperature $T_{sl}$ to liquidus temperature $T_{liq}$. $w_{fus} \; [kg/s]$ is given above and $c_{p_{cry, \; sol}} \; [J/(^\circ C \cdot kg)]$ is the heat capacity of solid cryolite. The time derivative of the side ledge temperature is given by:
\begin{equation}
    \Dot{T}_{sl} = \frac{Q_{liq-sl} - Q_{sl-wall} - E_{tc \; sol}}{m_{sl}c_{p_{cry,\; sol}}}
\end{equation}
$\Dot{T}_{sl} \; [^\circ C/s]$ is the temperature change in the side ledge, $Q_{liq-sl} \;[W]$ and $Q_{sl-wall} \; [W]$ is the heat in and out of the side ledge respectively. $m_{sl} \; [kg]$ is the mass of the side ledge, and $c_{p_{cry,\; sol}} \; [J/(^\circ C \cdot kg)]$ is the heat capacity of solid cryolite. There is no mass transfer through the \textbf{wall}. Therefore, the only energy transfer through this control volume is through heat transfer. The time derivative of the wall temperature $\Dot{T}_{wall} \; [~\circ C/s]$ is given by:
\begin{equation}
    \Dot{T}_{wall} = \frac{Q_{sl-wall} - Q_{wall - 0}}{m_{wall} c_{p_{wall}}}.
\end{equation}
$Q_{sl-wall} \; [W]$ is the heat from the side ledge to the wall, $Q_{wall - 0} \; [W]$ is the heat from the wall to the ambient, $m_{wall} \; [kg]$ is the mass og the wall and $c_{p_{wall}} \; [J/(^\circ C \cdot kg)]$ is the heat capacity of the wall.
\subsubsection{Liquidus temperature}


\subsubsection{Further simplifications in the simulation model}
In addition to assumptions and simplifications accounted for in the article, some additional simplifications are made in the simulation model. The reason for this is to simplify the analytical expression in the ODE's used to simulate the dynamics of the simulation model. The ODE's will still describe a complex nonlinear system, but comparing predictive models with the simulation models, and thus analysing the performance of the novel predictive models will be clearer. From the expression for $\Dot{T}_{bath}$ in (\ref{eq:T_dot_bath}), the terms $E_u, \; E_{sc}, \; E_{r_{Al}}$ and $E_{r_{bath}}$ are omitted. Thus, in the simulation model, the expression for $\Dot{T}_{bath}$ is given by:
\begin{equation}
    \Dot{T}_{bath, \; sim} = \frac{P_{el} - Q_{bath-sl} - E_{tc, \; liq}}{m_{bath}c_{p_{bath,\; liq}}}.
\end{equation}
This neglects some essential physical effects in the process. This is justified by the argument that the main purpose of this work is to evaluate the PGNN model on a complex nonlinear system, rather than simulating the dynamics of an aluminum electrolysis cell as good as possible.

